FAST: A Framework to Accelerate Super-Resolution Processing on Compressed Videos

State-of-the-art super-resolution (SR) algorithms require significant computational resources to achieve real-time throughput (e.g., 60Mpixels/s for HD video). This paper introduces FAST (Free Adaptive Super-resolution via Transfer), a framework to accelerate any SR algorithm applied to compressed videos. FAST exploits the temporal correlation between adjacent frames such that SR is only applied to a subset of frames; SR pixels are then transferred to the other frames. The transferring process has negligible computation cost as it uses information already embedded in the compressed video (e.g., motion vectors and residual). Adaptive processing is used to retain accuracy when the temporal correlation is not present (e.g., occlusions). FAST accelerates state-of-the-art SR algorithms by up to 15x with a visual quality loss of 0.2dB. FAST is an important step towards real-time SR algorithms for ultra-HD displays and energy constrained devices (e.g., phones and tablets).

==> 6_exploit_block_statistics.tex <==
\subsection{Exploit Block Statistics}
\label{sec:block_size}
To improve coding efficiency, the video encoder typically have special modes to reduce signaling information for the following scenarios: 
\begin{enumerate}
\item \textbf{Blocks with zero motion vector:} For pixels in zero motion vector blocks, FAST can directly \emph{copy} the same pixels from the previous frame without interpolation for motion compensation. This occurs for around 43\% of the pixels in the HEVC video dataset~\cite{jctvc2012test}. 
\item \textbf{Blocks with zero residual:} For pixels in such blocks, the bicubic interpolation on the residual can be \emph{skipped}. This occurs for around 82\% of the pixels in the HEVC video dataset~\cite{jctvc2012test}.
\end{enumerate}

FAST can exploit these \emph{copy} and \emph{skip} modes embedded in the compressed video to reduce the amount of interpolation and bicubic residual upsampling respectively. These modes are typically signaled with a flag syntax element in the encoded video that FAST can easily detect; for instance, the compressed video contains a bit for each block called the \textit{skip flag}, which indicates whether the residual is all zero or not. % By exploiting these special modes, FAST achieves an addition xxx speed up.


==> tables/blocks_vs_operations.tex <==
\def\tabularxcolumn#1{m{#1}}
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{tabularx}{1.1\columnwidth}{|c|Y|Y|Y|Y|Y|}
\hline
Block types & Anchored & Intra & \makecell{Inter\\zero\\ residual} & \makecell{Inter \\ zero mv} & Inter \\
\hline
\makecell{SR \\algorithm} & $\checkmark$ & & & &\\
\hline
\makecell{Bicubic\\ upsampling} & & $\checkmark$ & & $\checkmark$ & $\checkmark$\\
\hline
\makecell{Motion\\ compensation} & & & $\checkmark$ & & $\checkmark$ \\
\hline
\end{tabularx}
